Assessing the feasibility of near-ambient conditions superconductivity in the Lu-N-H system

The recent report of near-ambient superconductivity in nitrogen-doped lutetium hydrides (Lu-N-H) has generated a great interest. However, conflicting results have raised doubts regarding superconductivity. Here, we combine high-throughput crystal structure predictions with a fast predictor of the superconducting critical temperature ($T_c$) to shed light on the properties of Lu-N-H at 1 GPa. None of the predicted structures shows the potential to support high-temperature superconductivity and the inclusion of nitrogen favors the appearance of insulating phases. Despite the lack of near-ambient superconductivity, we consider alternative metastable templates and study their $T_c$ and dynamical stability including quantum anharmonic effects. The cubic Lu$_4$H$_{11}$N exhibits a high $T_c$ of 100 K at 20 GPa, a large increase compared to 30 K obtained in its parent LuH$_3$. Interestingly, it has a similar X-ray pattern to the experimentally observed one. The LaH$_{10}$-like LuH$_{10}$ and CaH$_6$-like LuH$_6$ become high-temperature superconductors at 175 GPa and 100 GPa, with $T_c$ of 286 K and 246 K, respectively. Our findings suggest that high-temperature superconductivity is not possible in stable phases at near-ambient pressure, but metastable high-$T_c$ templates exist at moderate and high pressures.

==> output-including-XRD-regardless-stability-240meV.tex <==
1fu\_Lu3H8N\_216 & 0.24 & $P\bar{3}m1$ & 0.26 & 0.31 & 13.94 & 75.03 \\
1fu\_Lu4H9\_138 & 0.21 & $P\bar{4}3m$ & 0.05 & 0.44 & -2.68 & 88.97 \\
1fu\_Lu4H9\_204 & 0.21 & $Cm$ & 0.05 & 0.42 & -4.52 & 86.67 \\
1fu\_Lu4H11N\_462 & 0.21 & $Cm$ & 0.40 & 0.21 & -4.95 & 52.28 \\
1fu\_Lu4H9\_63 & 0.13 & $Cmm2$ & 0.03 & 0.47 & -8.83 & 85.62 \\
1fu\_Lu4H11N\_34 & 0.20 & $Pm$ & 0.38 & 0.20 & -10.6 & 36.88 \\
2fu\_Lu4H11N\_570 & 0.14 & $P1$ & 0.18 & 0.25 & -11.59 & 93.23 \\
1fu\_Lu4H11N\_156 & 0.24 & $Pm$ & 0.34 & 0.20 & -12.94 & 43.05 \\
4fu\_Lu2H5N\_142 & 0.20 & $Imma$ & 0.32 & 0.22 & -14.74 & 43.34 \\
2fu\_Lu4H9\_155 & 0.20 & $P1$ & 0.03 & 0.42 & -15.73 & 41.71 \\
1fu\_Lu3H8N\_419 & 0.22 & $Amm2$ & 0.31 & 0.20 & -17.64 & 76.31 \\
1fu\_Lu4H7\_495 & 0.17 & $R3m$ & 0.04 & 0.42 & -17.88 & 64.48 \\
2fu\_Lu4H7\_242 & 0.17 & $Cmc2_1$ & 0.04 & 0.40 & -19.35 & 12.78 \\
2fu\_Lu4H9\_373 & 0.05 & $Pba2$ & 0.03 & 0.39 & -19.56 & 93.61 \\
1fu\_Lu4H9N\_150 & 0.22 & $Cm$ & 0.04 & 0.37 & -22.13 & 80.64 \\
2fu\_Lu4H7\_205 & 0.23 & $P\bar{1}$ & 0.02 & 0.45 & -23.48 & 68.34 \\
1fu\_Lu4H9\_22 & 0.01 & $C2/m$ & 0.04 & 0.33 & -25.1 & 99.25 \\
2fu\_Lu4H9\_34 & 0.02 & $Cm$ & 0.04 & 0.33 & -25.32 & 98.53 \\
1fu\_Lu4H9\_213 & 0.01 & $Cmmm$ & 0.04 & 0.34 & -25.58 & 99.07 \\
2fu\_Lu4H9\_231 & 0.01 & $P2_1/m$ & 0.04 & 0.34 & -26.0 & 99.48 \\
1fu\_Lu4H9\_99 & 0.16 & $Cmm2$ & 0.04 & 0.34 & -26.2 & 63.02 \\
1fu\_Lu4H9\_86 & 0.05 & $C2/m$ & 0.04 & 0.32 & -26.89 & 99.26 \\
1fu\_Lu4H9\_114 & 0.12 & $P\bar{1}$ & 0.03 & 0.35 & -27.51 & 84.71 \\
1fu\_Lu4H9\_190 & 0.11 & $R3m$ & 0.05 & 0.30 & -28.28 & 62.05 \\
1fu\_Lu4H7N\_359 & 0.23 & $Fmm2$ & 0.04 & 0.37 & -28.4 & 69.44 \\
2fu\_Lu4H7\_467 & 0.17 & $C2/m$ & 0.02 & 0.42 & -29.02 & 99.45 \\
1fu\_Lu4H7\_312 & 0.18 & $Cm$ & 0.02 & 0.41 & -29.28 & 75.27 \\
2fu\_Lu4H7\_98 & 0.21 & $C2$ & 0.03 & 0.37 & -29.47 & 75.79 \\
1fu\_Lu4H7\_415 & 0.19 & $P4mm$ & 0.02 & 0.42 & -29.63 & 69.74 \\
1fu\_Lu4H9N\_202 & 0.14 & $P2/m$ & 0.26 & 0.18 & -29.73 & 23.46 \\
2fu\_Lu4H7\_340 & 0.22 & $Pbam$ & 0.03 & 0.39 & -30.11 & 40.43 \\
2fu\_Lu4H11N\_574 & 0.15 & $P1$ & 0.04 & 0.31 & -30.63 & 72.06 \\
2fu\_Lu4H9\_12 & 0.15 & $Cm$ & 0.03 & 0.32 & -31.37 & 94.71 \\
1fu\_Lu4H7\_166 & 0.20 & $Amm2$ & 0.02 & 0.45 & -31.62 & 97.01 \\
2fu\_Lu4H7\_223 & 0.20 & $Cc$ & 0.03 & 0.36 & -31.65 & 13.44 \\
2fu\_Lu4H9\_64 & 0.15 & $P2_1$ & 0.03 & 0.33 & -31.81 & 61.22 \\
1fu\_Lu4H7\_373 & 0.21 & $C2/m$ & 0.03 & 0.37 & -31.91 & 56.22 \\
2fu\_Lu4H7\_51 & 0.19 & $P4/mmm$ & 0.02 & 0.43 & -32.23 & 68.09 \\
1fu\_Lu4H9\_208 & 0.01 & $Pm\bar{3}m$ & 0.03 & 0.32 & -32.29 & 99.75 \\
2fu\_Lu4H9\_233 & 0.01 & $Cmmm$ & 0.04 & 0.30 & -32.3 & 98.97 \\
2fu\_Lu4H9\_190 & 0.01 & $Pmmm$ & 0.03 & 0.32 & -32.51 & 98.92 \\
2fu\_Lu4H9\_252 & 0.01 & $P\bar{1}$ & 0.04 & 0.30 & -32.61 & 99.16 \\
1fu\_Lu4H9\_139 & 0.06 & $Pmmm$ & 0.03 & 0.32 & -32.68 & 98.66 \\
2fu\_Lu4H7\_238 & 0.22 & $Cm$ & 0.03 & 0.36 & -32.7 & 28.71 \\
1fu\_Lu4H9\_175 & 0.01 & $Pm\bar{3}m$ & 0.03 & 0.32 & -32.85 & 99.12 \\
2fu\_Lu3H8N\_351 & 0.21 & $C2/m$ & 0.28 & 0.16 & -32.92 & 51.18 \\
2fu\_Lu4H9\_23 & 0.16 & $Cmmm$ & 0.03 & 0.34 & -32.97 & 75.46 \\
2fu\_Lu4H7\_391 & 0.04 & $Pc$ & 0.03 & 0.35 & -33.55 & 97.01 \\
2fu\_Lu4H7\_62 & 0.08 & $Fmm2$ & 0.03 & 0.35 & -33.57 & 98.19 \\
1fu\_Lu4H9\_215 & 0.01 & $Pmmm$ & 0.03 & 0.31 & -33.72 & 98.52 \\
1fu\_Lu4H7\_204 & 0.06 & $R\bar{3}m$ & 0.02 & 0.39 & -33.8 & 96.55 \\
1fu\_Lu4H9\_182 & 0.01 & $Pmmm$ & 0.03 & 0.31 & -34.12 & 98.91 \\
2fu\_Lu4H9\_221 & 0.11 & $Pc$ & 0.03 & 0.30 & -34.26 & 61.50 \\
2fu\_Lu4H7\_202 & 0.21 & $Cmc2_1$ & 0.03 & 0.33 & -34.3 & 43.18 \\
2fu\_Lu4H7\_149 & 0.09 & $P2_1/m$ & 0.03 & 0.33 & -34.5 & 98.41 \\
2fu\_Lu4H7\_274 & 0.18 & $Pmmm$ & 0.03 & 0.36 & -34.68 & 97.59 \\
2fu\_Lu4H7\_66 & 0.03 & $Cmcm$ & 0.03 & 0.34 & -34.7 & 97.52 \\
1fu\_Lu4H7\_75 & 0.18 & $C2$ & 0.02 & 0.36 & -34.77 & 99.04 \\
2fu\_Lu4H7\_497 & 0.23 & $Pmn2_1$ & 0.03 & 0.34 & -35.0 & 45.59 \\
2fu\_Lu4H9\_430 & 0.13 & $Cm$ & 0.03 & 0.30 & -35.65 & 95.81 \\
1fu\_Lu4H7\_318 & 0.12 & $Amm2$ & 0.03 & 0.34 & -36.45 & 97.97 \\
1fu\_Lu4H7N\_78 & 0.24 & $P\bar{4}2m$ & 0.03 & 0.34 & -36.47 & 67.72 \\
1fu\_Lu4H7\_478 & 0.04 & $Amm2$ & 0.03 & 0.34 & -36.53 & 99.15 \\
1fu\_Lu4H7\_417 & 0.03 & $P\bar{4}3m$ & 0.02 & 0.35 & -36.77 & 97.87 \\
2fu\_Lu4H9\_46 & 0.14 & $P1$ & 0.04 & 0.27 & -36.96 & 15.41 \\
1fu\_Lu4H7\_32 & 0.16 & $Cmmm$ & 0.02 & 0.39 & -36.98 & 77.44 \\
2fu\_Lu4H7\_140 & 0.18 & $P6_3mc$ & 0.03 & 0.33 & -37.09 & 12.13 \\
2fu\_Lu4H7\_169 & 0.16 & $P\bar{1}$ & 0.02 & 0.34 & -37.64 & 83.42 \\
2fu\_Lu4H7\_375 & 0.09 & $Cmc2_1$ & 0.03 & 0.33 & -37.66 & 95.62 \\
1fu\_Lu4H9\_54 & 0.16 & $C2/m$ & 0.03 & 0.29 & -37.73 & 77.29 \\
1fu\_Lu4H11N\_161 & 0.23 & $Cm$ & 0.13 & 0.18 & -37.94 & 66.75 \\
1fu\_Lu4H7\_64 & 0.07 & $Cm$ & 0.03 & 0.31 & -37.98 & 97.45 \\
2fu\_Lu4H9\_128 & 0.23 & $C2$ & 0.04 & 0.26 & -38.11 & 45.05 \\
1fu\_Lu4H7\_288 & 0.16 & $Amm2$ & 0.02 & 0.35 & -38.25 & 65.62 \\
1fu\_Lu4H7\_118 & 0.20 & $Cm$ & 0.03 & 0.33 & -38.38 & 64.77 \\
1fu\_Lu4H7\_313 & 0.19 & $Amm2$ & 0.03 & 0.32 & -38.59 & 58.34 \\
2fu\_Lu4H7\_323 & 0.24 & $C2$ & 0.03 & 0.33 & -38.65 & 35.99 \\
1fu\_Lu4H11N\_124 & 0.22 & $C2/m$ & 0.04 & 0.26 & -38.83 & 67.27 \\
1fu\_Lu4H7\_467 & 0.23 & $P\bar{4}m2$ & 0.02 & 0.39 & -38.88 & 59.39 \\
2fu\_Lu4H9\_152 & 0.23 & $Cm$ & 0.04 & 0.27 & -38.96 & 48.52 \\
1fu\_Lu4H7\_185 & 0.16 & $Cmmm$ & 0.02 & 0.38 & -39.04 & 75.89 \\
1fu\_Lu4H7\_138 & 0.16 & $Cmmm$ & 0.02 & 0.38 & -39.04 & 76.86 \\
1fu\_Lu4H7\_96 & 0.16 & $Cmmm$ & 0.02 & 0.38 & -39.3 & 77.47 \\
1fu\_Lu4H7N\_222 & 0.10 & $Cm$ & 0.03 & 0.34 & -39.36 & 39.69 \\
2fu\_Lu4H9\_401 & 0.02 & $P4/mmm$ & 0.04 & 0.26 & -39.37 & 99.12 \\
2fu\_Lu4H7\_63 & 0.17 & $Cmc2_1$ & 0.03 & 0.32 & -39.55 & 62.64 \\
2fu\_Lu4H9\_475 & 0.14 & $Pmn2_1$ & 0.04 & 0.26 & -39.76 & 24.51 \\
2fu\_Lu4H7\_59 & 0.24 & $P1$ & 0.02 & 0.36 & -39.81 & 46.70 \\
2fu\_Lu4H9\_203 & 0.16 & $P2/c$ & nan & 0.27 & -39.93 & 52.38 \\
2fu\_Lu4H9\_192 & 0.22 & $Cm$ & 0.04 & 0.25 & -40.27 & 36.96 \\
1fu\_Lu4H7N\_405 & 0.10 & $Cm$ & 0.04 & 0.31 & -40.57 & 44.22 \\
1fu\_Lu4H7\_29 & 0.16 & $P1$ & 0.02 & 0.33 & -40.67 & 68.36 \\
2fu\_Lu4H9\_44 & 0.14 & $Cm$ & 0.04 & 0.26 & -40.71 & 72.21 \\
2fu\_Lu4H7\_58 & 0.20 & $Cc$ & 0.02 & 0.32 & -41.01 & 54.10 \\
1fu\_Lu4H7N\_358 & 0.10 & $R3m$ & 0.02 & 0.36 & -41.32 & 68.35 \\
2fu\_Lu4H9\_225 & 0.20 & $P1$ & 0.03 & 0.26 & -41.51 & 97.85 \\
3fu\_Lu2H5N\_311 & 0.19 & $P1$ & 0.04 & 0.26 & -41.68 & 44.71 \\
2fu\_Lu4H9\_138 & 0.08 & $Pmm2$ & 0.03 & 0.26 & -41.69 & 99.04 \\
1fu\_Lu4H8N\_326 & 0.18 & $P\bar{4}m2$ & 0.03 & 0.30 & -41.74 & 86.35 \\
2fu\_Lu4H7\_346 & 0.12 & $Pc$ & 0.02 & 0.32 & -41.82 & 98.34 \\
1fu\_Lu4H8N\_491 & 0.12 & $Cm$ & 0.05 & 0.26 & -41.95 & 82.29 \\
2fu\_Lu4H7\_39 & 0.12 & $Cmmm$ & 0.02 & 0.31 & -41.95 & 79.61 \\
2fu\_Lu4H9\_436 & 0.13 & $Cc$ & 0.04 & 0.25 & -42.11 & 14.54 \\
1fu\_Lu4H8N\_444 & 0.15 & $Amm2$ & 0.04 & 0.28 & -42.3 & 69.01 \\
2fu\_Lu4H9\_117 & 0.23 & $Pm$ & 0.03 & 0.26 & -42.35 & 69.30 \\
1fu\_Lu4H8N\_141 & 0.20 & $Cm$ & 0.03 & 0.31 & -42.57 & 58.82 \\
2fu\_Lu4H9\_184 & 0.10 & $I4mm$ & 0.02 & 0.28 & -42.75 & 22.18 \\
2fu\_Lu4H9\_380 & 0.10 & $Cmcm$ & 0.03 & 0.26 & -43.49 & 95.13 \\
1fu\_Lu4H7\_367 & 0.19 & $P1$ & 0.03 & 0.28 & -43.5 & 48.26 \\
2fu\_Lu4H9\_113 & 0.15 & $P1$ & 0.03 & 0.25 & -43.84 & 58.26 \\
1fu\_Lu4H9N\_216 & 0.21 & $P1$ & 0.03 & 0.26 & -44.17 & 49.05 \\
1fu\_Lu4H7\_232 & 0.14 & $R3m$ & 0.02 & 0.31 & -44.58 & 63.09 \\
1fu\_Lu4H7\_81 & 0.17 & $Cm$ & 0.02 & 0.31 & -44.59 & 57.65 \\
1fu\_Lu4H9\_167 & 0.01 & $I4/mmm$ & 0.03 & 0.25 & -44.64 & 98.97 \\
2fu\_Lu4H9\_299 & 0.01 & $I4/mmm$ & 0.03 & 0.25 & -44.64 & 98.92 \\
1fu\_Lu4H7\_386 & 0.19 & $Pmm2$ & 0.02 & 0.32 & -44.88 & 60.30 \\
1fu\_Lu4H8N\_5 & 0.07 & $R\bar{3}m$ & 0.03 & 0.27 & -44.97 & 51.47 \\
1fu\_Lu4H7N\_471 & 0.15 & $Pmm2$ & 0.03 & 0.28 & -45.06 & 67.44 \\
2fu\_Lu4H9\_191 & 0.15 & $Cmm2$ & 0.04 & 0.23 & -45.06 & 76.30 \\
1fu\_Lu4H7\_44 & 0.19 & $C2$ & 0.02 & 0.30 & -45.25 & 58.91 \\
2fu\_Lu4H9\_210 & 0.24 & $P2_1$ & 0.03 & 0.25 & -45.38 & 84.27 \\
2fu\_Lu4H9\_111 & 0.10 & $Cc$ & 0.03 & 0.24 & -45.43 & 91.48 \\
1fu\_Lu4H7N\_446 & 0.23 & $Cm$ & 0.05 & 0.25 & -45.93 & 74.54 \\
1fu\_Lu4H7N\_166 & 0.15 & $P1$ & 0.04 & 0.26 & -45.95 & 27.14 \\
2fu\_Lu3H8N\_4 & 0.23 & $P1$ & 0.04 & 0.22 & -45.95 & 71.09 \\
1fu\_Lu4H9\_235 & 0.15 & $Cmm2$ & 0.03 & 0.24 & -45.96 & 73.67 \\
2fu\_Lu4H7\_456 & 0.22 & $Cm$ & 0.02 & 0.28 & -46.0 & 58.31 \\
2fu\_Lu2H5N\_142 & 0.23 & $Pma2$ & 0.20 & 0.14 & -46.34 & 8.76 \\
1fu\_Lu4H9\_194 & 0.11 & $R\bar{3}m$ & 0.02 & 0.26 & -46.36 & 91.31 \\
1fu\_Lu4H11N\_150 & 0.16 & $P1$ & 0.03 & 0.25 & -46.41 & 49.40 \\
1fu\_Lu4H9N\_10 & 0.21 & $P3m1$ & 0.04 & 0.24 & -46.57 & 37.17 \\
1fu\_Lu4H9\_6 & 0.16 & $P1$ & 0.04 & 0.22 & -46.88 & 64.86 \\
2fu\_Lu3H8N\_116 & 0.20 & $P1$ & 0.03 & 0.24 & -47.27 & 49.77 \\
2fu\_Lu4H9\_336 & 0.22 & $Pmc2_1$ & 0.04 & 0.22 & -47.54 & 74.96 \\
1fu\_Lu4H7\_223 & 0.20 & $P2$ & 0.02 & 0.28 & -47.64 & 73.17 \\
2fu\_Lu4H9\_364 & 0.24 & $Cc$ & 0.04 & 0.21 & -48.79 & 94.71 \\
1fu\_Lu4H9N\_136 & 0.04 & $P3m1$ & 0.31 & 0.11 & -48.99 & 13.12 \\
1fu\_Lu4H7\_340 & 0.10 & $Pmmm$ & 0.02 & 0.30 & -49.15 & 98.19 \\
2fu\_Lu4H9\_323 & 0.19 & $C2/m$ & 0.03 & 0.23 & -49.35 & 53.14 \\
1fu\_Lu4H11N\_251 & 0.19 & $Cm$ & 0.05 & 0.19 & -49.69 & 66.42 \\
1fu\_Lu4H8N\_489 & 0.23 & $Cm$ & 0.03 & 0.24 & -50.02 & 68.51 \\
1fu\_Lu4H7\_378 & 0.14 & $Cmm2$ & 0.02 & 0.27 & -50.04 & 79.79 \\
1fu\_Lu4H7\_325 & 0.24 & $Amm2$ & 0.02 & 0.25 & -50.53 & 71.05 \\
1fu\_Lu4H8N\_436 & 0.16 & $P\bar{4}$ & 0.04 & 0.22 & -50.6 & 11.86 \\
1fu\_Lu2H5N\_194 & 0.17 & $Cm$ & 0.39 & 0.10 & -50.89 & 62.99 \\
2fu\_Lu4H9\_335 & 0.22 & $P4/m$ & 0.02 & 0.23 & -51.35 & 13.51 \\
1fu\_Lu4H7\_307 & 0.12 & $P2$ & 0.02 & 0.25 & -51.75 & 83.52 \\
2fu\_Lu4H11N\_548 & 0.22 & $P1$ & 0.03 & 0.21 & -51.94 & 73.65 \\
1fu\_Lu4H7\_228 & 0.21 & $Pm$ & 0.02 & 0.25 & -51.95 & 52.84 \\
2fu\_Lu4H11N\_595 & 0.16 & $P1$ & 0.04 & 0.19 & -52.22 & 55.28 \\
1fu\_Lu4H7N\_375 & 0.17 & $Cm$ & 0.02 & 0.27 & -52.44 & 42.71 \\
1fu\_Lu4H7N\_280 & 0.19 & $P1$ & 0.03 & 0.23 & -52.51 & 42.08 \\
1fu\_Lu4H7N\_325 & 0.20 & $Amm2$ & 0.04 & 0.22 & -52.52 & 96.86 \\
1fu\_Lu4H7N\_11 & 0.11 & $Cm$ & 0.03 & 0.24 & -52.56 & 91.97 \\
1fu\_Lu4H8N\_308 & 0.15 & $Pm$ & 0.03 & 0.22 & -52.9 & 26.63 \\
1fu\_Lu4H8N\_9 & 0.21 & $P4mm$ & 0.04 & 0.21 & -53.22 & 64.27 \\
2fu\_Lu3H8N\_186 & 0.22 & $P6_3/mmc$ & 0.06 & 0.16 & -53.34 & 65.81 \\
1fu\_Lu4H7\_455 & 0.15 & $Pmm2$ & 0.02 & 0.23 & -53.65 & 94.68 \\
1fu\_Lu4H8N\_494 & 0.14 & $Amm2$ & 0.03 & 0.23 & -53.77 & 28.24 \\
2fu\_Lu4H9\_332 & 0.23 & $C2$ & 0.03 & 0.19 & -53.89 & 60.13 \\
1fu\_Lu4H9N\_385 & 0.17 & $Pm$ & 0.04 & 0.19 & -53.99 & 71.40 \\
1fu\_Lu4H8N\_198 & 0.10 & $Pmm2$ & 0.03 & 0.22 & -54.2 & 72.35 \\
1fu\_Lu4H9\_216 & 0.15 & $P\bar{6}m2$ & 0.02 & 0.21 & -55.28 & 42.84 \\
1fu\_Lu4H7\_379 & 0.20 & $Pm$ & 0.02 & 0.22 & -55.31 & 88.22 \\
2fu\_Lu4H9\_444 & 0.24 & $P2_1/m$ & 0.03 & 0.19 & -55.58 & 60.56 \\
1fu\_Lu4H8N\_410 & 0.14 & $Cm$ & 0.04 & 0.19 & -55.64 & 76.18 \\
1fu\_Lu4H9\_52 & 0.16 & $Amm2$ & 0.02 & 0.20 & -55.91 & 60.98 \\
1fu\_Lu4H8N\_105 & 0.07 & $Pm$ & 0.03 & 0.21 & -56.18 & 74.46 \\
1fu\_Lu4H8N\_46 & 0.14 & $Pm$ & 0.03 & 0.20 & -56.19 & 27.61 \\
1fu\_Lu4H7N\_377 & 0.15 & $Cm$ & 0.03 & 0.20 & -56.47 & 21.50 \\
3fu\_Lu2H5N\_89 & 0.23 & $C2$ & 0.03 & 0.20 & -56.82 & 57.28 \\
1fu\_Lu4H9N\_83 & 0.19 & $Pm$ & 0.04 & 0.17 & -56.92 & 81.91 \\
1fu\_Lu4H7N\_491 & 0.14 & $P1$ & 0.03 & 0.21 & -57.5 & 84.14 \\
1fu\_Lu4H9\_129 & 0.15 & $Imm2$ & 0.03 & 0.17 & -57.64 & 14.80 \\
1fu\_Lu4H7N\_172 & 0.17 & $P1$ & 0.03 & 0.21 & -57.7 & 83.10 \\
2fu\_Lu4H9\_92 & 0.22 & $Cc$ & 0.03 & 0.17 & -57.74 & 45.77 \\
2fu\_Lu4H7N\_206 & 0.19 & $P4_2mc$ & 0.03 & 0.21 & -57.84 & 27.93 \\
1fu\_Lu4H7N\_48 & 0.23 & $Pm$ & 0.03 & 0.19 & -58.03 & 63.99 \\
2fu\_Lu4H9\_67 & 0.14 & $P4_2/nmc$ & 0.02 & 0.20 & -58.06 & 40.45 \\
2fu\_Lu4H9\_115 & 0.19 & $C2/c$ & 0.04 & 0.15 & -58.36 & 33.31 \\
1fu\_Lu4H7N\_488 & 0.17 & $Cm$ & 0.02 & 0.22 & -58.37 & 67.76 \\
1fu\_Lu4H7N\_49 & 0.10 & $I\bar{4}2m$ & 0.03 & 0.20 & -58.61 & 59.77 \\
1fu\_Lu4H8N\_334 & 0.08 & $Cm$ & 0.03 & 0.18 & -58.69 & 68.93 \\
1fu\_Lu4H8N\_72 & 0.22 & $Pm$ & 0.03 & 0.18 & -58.99 & 64.08 \\
4fu\_Lu2H5N\_206 & 0.20 & $P1$ & 0.03 & 0.17 & -59.1 & 61.21 \\
1fu\_Lu4H8N\_150 & 0.14 & $Cm$ & 0.02 & 0.19 & -59.37 & 32.61 \\
1fu\_Lu4H7N\_420 & 0.13 & $Pmm2$ & 0.03 & 0.19 & -59.45 & 65.32 \\
1fu\_Lu4H8N\_37 & 0.16 & $Cmmm$ & 0.02 & 0.21 & -59.55 & 65.12 \\
1fu\_Lu4H8N\_224 & 0.07 & $Amm2$ & 0.03 & 0.18 & -59.69 & 46.12 \\
1fu\_Lu3H8N\_417 & 0.23 & $Cm$ & 0.04 & 0.14 & -60.17 & 57.58 \\
1fu\_Lu4H8N\_196 & 0.18 & $Cm$ & 0.03 & 0.18 & -60.58 & 14.69 \\
1fu\_Lu4H7N\_107 & 0.21 & $C2$ & 0.03 & 0.18 & -60.64 & 66.81 \\
1fu\_Lu4H7N\_372 & 0.15 & $P4mm$ & 0.03 & 0.19 & -60.64 & 52.78 \\
1fu\_Lu4H8N\_216 & 0.16 & $Cm$ & 0.03 & 0.17 & -61.08 & 60.05 \\
2fu\_Lu4H8N\_326 & 0.10 & $P4_2/nmc$ & 0.02 & 0.18 & -61.3 & 67.61 \\
1fu\_Lu4H8N\_119 & 0.13 & $P1$ & 0.03 & 0.17 & -61.35 & 64.41 \\
1fu\_Lu4H7N\_424 & 0.09 & $P\bar{4}3m$ & 0.02 & 0.19 & -61.7 & 61.73 \\
2fu\_Lu4H9\_420 & 0.04 & $Cmcm$ & 0.03 & 0.15 & -62.03 & 93.12 \\
3fu\_Lu2H5N\_336 & 0.14 & $P\bar{3}m1$ & 0.03 & 0.16 & -62.78 & 46.56 \\
1fu\_Lu4H7N\_293 & 0.22 & $C2$ & 0.03 & 0.16 & -63.08 & 49.69 \\
1fu\_Lu4H7N\_190 & 0.21 & $Cm$ & 0.02 & 0.17 & -63.73 & 65.93 \\
1fu\_Lu4H8N\_83 & 0.18 & $Cm$ & 0.03 & 0.15 & -64.17 & 57.73 \\
1fu\_Lu4H7N\_494 & 0.15 & $Cm$ & 0.02 & 0.16 & -64.6 & 63.68 \\
2fu\_Lu2H5N\_194 & 0.08 & $P1$ & 0.02 & 0.14 & -66.45 & 63.50 \\
1fu\_Lu4H9N\_167 & 0.22 & $R3m$ & 0.03 & 0.13 & -66.49 & 42.43 \\
1fu\_Lu4H7N\_495 & 0.22 & $Cm$ & 0.02 & 0.14 & -67.18 & 23.42 \\
1fu\_Lu4H7N\_67 & 0.02 & $R\bar{3}m$ & 0.03 & 0.06 & -76.61 & 53.46 \\
1fu\_Lu2H5N\_439 & 0.21 & $Cm$ & 0.28 & nan & nan & 61.86 \\
1fu\_Lu3H8N\_431 & 0.13 & $Cm$ & 0.04 & nan & nan & 86.07 \\
1fu\_Lu4H11N\_196 & 0.17 & $C2$ & 0.39 & nan & nan & 60.82 \\
1fu\_Lu4H8N\_175 & 0.13 & $C2$ & 0.03 & nan & nan & 81.56 \\
1fu\_Lu4H9\_127 & 0.20 & $Cm$ & 0.03 & nan & nan & 61.62 \\
1fu\_Lu4H9\_74 & 0.01 & $C2/m$ & 0.04 & nan & nan & 99.19 \\
2fu\_Lu4H9\_63 & 0.02 & $I4/mmm$ & 0.04 & nan & nan & 99.24 \\

